Improving Blockchain Consistency Bound by Assigning Weights to Random Blocks

Blockchains based on the celebrated Nakamoto consensus protocol have shown promise in several applications, including cryptocurrencies. However, these blockchains have inherent scalability limits caused by the protocol's consensus properties. In particular, the \emph{consistency} property demonstrates a tight trade-off between block production speed and the system's security in terms of resisting adversarial attacks. This paper proposes a novel method, Ironclad, that improves blockchain consistency bound by assigning a different weight to randomly selected blocks. We apply our method to the original Nakamoto protocol and rigorously prove that such a combination can improve the consistency bound significantly by analyzing the fundamental consensus properties. Such an improvement enables a much faster block production rate than the original Nakamoto protocol under the same security guarantee with the same proportion of malicious mining power (see Figure 1).

==> analysis/discussion_parameters.tex <==


\subsection{The Selection of Parameters}
\label{subsec: selection of q}
% The parameters in the protocol can be divided into two categories: 
% those that should be given as prior, such as delay $\Delta$ and honest mining power $p_h$, 
% and those that can be artificially selected, such as the weight parameter $\theta$ and the relative difficulty parameter $q$. 

% \par \smallskip
\noindent \textbf{A Lower Bound of $\theta$.}
The example in \cref{fig: high-diff block} shows how \BB s lead to consensus by dominating the competing \SB s (corresponding to $\sigma_4$) due to their larger weight.
This outcome requires that $\theta$ be larger than the number of competing \SB s within the preceding and following $\Delta$ time slots at creating such an \BB\ (corresponding to $\sigma_4$).
Hence a naive lower bound is $2\Delta$, which is too large in practice.
The weight parameter $\theta$, jointly with the \qnames $q$, should be a hyperparameter to allow different choices and optimization. 
We can trade off the value of $\theta$ and the requirement holding probability.
We first construct the upper confidence bound of the number of \SB s in $\sigma_4$. 
% However, it is too strict since $\Delta$ is usually very large for approximation.
% In \cite{asynchronous_networks,better_method} $\Delta \approx 11.2s$ is divided into $10^{13}$ rounds, 
% and each round lasts $1.12\times 10^{-12}s$ to approximate the mining process precisely.
% The weight parameter $\theta$, independent of difficulty, is a hyperparameter with freedom by design. 
% A naive lower bound $2\Delta$ is too large in practice. 
% To establish a smaller lower bound of $\theta$, 
% we can first construct an upper confidence bound of the number of \SB s in $\Delta$ time slots. 
% By selecting a proper $\theta$, 
% we can ignore some transitions in the Markov chain with negligible probability for simplification.

\begin{mylem}
    \label{lem: setting theta}
    The probability that the number of \SB s $Y$ in the pattern $\sigma_4$ exceeding $\theta$ decays exponentially as $\theta$ grows. More precisely,
    $$
    \prob{Y\geq \theta} \leq \exp\left(-\frac{q_h\Delta \delta^2}{(1-q_H)(2+\delta)}\right),
    $$
    where $\delta = (\frac{1-q_H}{  q_h\Delta})\theta-1$.
\end{mylem}

% JZ: move the proof to appendix.
\begin{myproof}
The probability for `h' to appear in each time slot is $q_h$
Conditioning on pattern $\sigma_4$, the number of symbol `h' $Y$ follows a binomial distribution with parameters $\Delta$ and $q_h/(1-q_H)$. 
We can obtain the inequality by applying the Chernoff's inequality to $Y$.
\end{myproof}

% \begin{myrem}\label{rem:lower bound for theta}
% The probability inequality results in the lower bound of $\theta$. 
% For a given tolerance probability $\epsilon$, 
% we can make the probability of the event $\{Y\geq\theta\}$ less than $\epsilon$ if we choose $\theta$ satisfying 
% \begin{equation*}
% \begin{array}{rcl}
% \theta &>& \frac{q_h\Delta}{1-q_H} + \frac{1}{2} \ln \epsilon^{-1} \\
% & + & \frac{1}{2}\sqrt{  (\ln \epsilon^{-1})^2 +8 q_h\Delta (1-q_H)^{-1}     \ln \epsilon^{-1}    }.
% \end{array}
% \end{equation*}
To satisfy the requirement with probability $1-\epsilon$, we can leverage \cref{lem: setting theta} to construct an lower confidence bound of $\theta$ as
\begin{equation}
    \label{eq:theta lower bound}
	\underline{\theta} := \frac{2 q_h\Delta}{1-q_H} -  \ln \epsilon 
	+ \sqrt{(\ln \epsilon)^2 - \frac{8 q_h\Delta}{1-q_H}   \ln \epsilon}.
\end{equation}

% We are also interested in the state transition $S_1\myto{\sigma_4}S_0$ since it produces the opportunity for honest parties to reach an agreement. 
% The \cref{fig: high-diff block} shows how \BB s contribute to the consistency. 
% In order to ignore the effect of \SB s on \BB s, 
% it requires that the number of `h' before `H' is less than $\theta$ in previous $\Delta$ time slots. 
% Clearly, the distribution is the same as $Y$ so 
% \begin{equation*}
% \begin{array}{rcl}
% \theta > \underline{\theta} &:=& \frac{2 q_h\Delta}{1-q_H} +  \ln \epsilon^{-1} \\
% &+& \sqrt{  (\ln \epsilon^{-1})^2 +8 q_h\Delta (1-q_H)^{-1}     \ln \epsilon^{-1}    }
% \end{array}
% \end{equation*}
% by model assumptions.
% \end{myrem}


% If 
% $$
% \theta >   {2 p_h\Delta} +  \ln \epsilon^{-1} +
% \sqrt{  (\ln \epsilon^{-1})^2 +8 p_h\Delta   \ln \epsilon^{-1}   },
% $$
% then we do not need to consider the effect of $q$.

In \cite{asynchronous_networks,better_method}, $p_h = 10^{-13}$, $\Delta = 10^{13} $ time slots,
which corresponds to the case where the average time between two honest blocks is 10 seconds.
By setting a significance level $\epsilon = 10^{-10}$,
we can get $\theta \geq 51.8$, $\forall q\in(0,1)$, 
which is a mild requirement for $\theta$ compared with $2\Delta$.

% since this conservative lower bound is based on the total number of \SB s within $2\Delta$ time slots, 
% and actually $\theta$ only needs to be larger than the maximum of the total number of \SB s mined in a single chain.
% Therefore, in the following analysis, we assume that $\theta$ is large enough to ignore rarely happening transitions related with \BB s, such as $S_2 \to S_1$.

% We have obtained a lower bound of $\theta$ from the assumption that 
% the number of \SB s produced in $2\Delta$ rounds will not exceed $\theta$ with high probability. 
% The upper bound of $\theta$ will be derived from security analysis in \cref{section: Security}. 
% $\theta$ cannot be too large in order to defend against consensus attacks effectively. 
% Otherwise, it will make the block confirmation time too long.

\par \smallskip
\noindent \textbf{Optimal $q^*$.}
Another parameter in Ironclad is $q$, which controls the frequency of \BB s among all valid blocks.
According to \cref{thm: Consistency}, consistency is satisfied for $\beta<\alpha$, or equivalently,  
$$
\frac{p_a}{p_h} < \frac{\alpha}{p_h(1-q+\theta q)}.
$$
To select a reasonable $q$, we define the tolerance ratio of mining power between the adversary and honest parties. 
\begin{mydef}[Tolerance Ratio]
    \label{def: tolerance ratio}
The tolerance ratio $\mathcal{A}$ is defined as
$$
\mathcal{A} = \frac{\alpha}{p_h(1-q+\theta q)}.
$$
\end{mydef}
The analytical expression for the tolerance ratio is shown in \cref{eq:expression of A}.
In order to deal with it mathematically, we also derive a close approximation $\tilde{\mathcal{A}}$ in \eqref{eq:A tilde}.
We show that $\tilde{\mathcal{A}}$ fits $\mathcal{A}$ well in \cref{fig:adv_ratio in theory}.
We find three interesting properties of $\mathcal{A}$,
which reveals some unique features of our method.
\begin{mythm}
  \label{prop:adversary ratio properties}
  For any $p_h$, $\Delta$ and $\theta\geq \max(\underline\theta,1)$, 
\begin{enumerate}
    \item the maximizer $q^*$ for $\mathcal{A}$ exists in $(0,1)$;
    \item a unique maximizer $q^*(\theta)$ of $\tilde{\mathcal{A}}$ exists in $(0,1)$. Moreover, $q^*(\theta)$ decreases in $\theta$;
    \item the optimal value $\mathcal{A}^*_{\theta}$ of $\mathcal{A}$ for each $\theta$ increases in $\theta$.
\end{enumerate}
\end{mythm}

The intuition of the proof, which is in \cref{appendix: proof of A}, can be explained using the first chart in \cref{fig:adv_ratio in theory}. 
The system consensus benefits (tolerance ratio $\mathcal{A}$ increases) from increasing $q$ when $q$ is small. 
% JZ: It is non-monotonicity?
% monotonicity of $\mathcal{A}$
This is because \BB s can effectively reduce the forks caused by \SB s. 
However, when $q$ exceeds a certain threshold $q^*$, $\mathcal{A}$ starts to decrease because the competition among \BB s themselves becomes the main issue as \SB s become less.

The unimodality of tolerance ratio in $q$ provides useful insights. 
If we fix $p_h$, $\Delta$ and $\theta$, there will exist a non-trivial maximizer $q^*$ for it.
Therefore, we can obtain the optimal $q^*$ by maximizing $\mathcal{A}$ for each $\theta$, which can be numerically solved.
The second chart of \cref{fig:adv_ratio in theory} illustrates the corresponding results for specific $p_h$ and $\Delta$ in the Ethereum setting.
We find a decreasing trend for $q^*$ as $\theta$ grows, which conforms to our intuition.
The approximation result for $q^*(\theta)$ also explains the intuition mathematically.
It is obvious that the approximation curve fits the sample points very well.

% JZ: The following sentence seems unnecessary. 
% Now, we can study the optimal objective value. 
% \bgmlover{has been defined before}
% For notation brevity, 
% denote $\mathcal{A}^*_{\theta}$ as the optimal object value for a specific $\theta$.
% It is observable that $\mathcal{A}$ is increasing in $\theta$.
% Therefore, it is straightforward that $\mathcal{A}^*_{\theta}$ is increasing in $\theta$.        
The third property is depicted in the third chart of \cref{fig:adv_ratio in theory}.
The mining power gap in the original Nakamoto protocol is $p_h-p_a$, 
and it is scaled up to be $(p_h-p_a)(1-q+q\theta)$ in Nakamoto+\protocol\ due to the effect of \BB s, 
which indicates that the new one can tolerate more adversarial mining power. 

% The newly defined quantity is equivalent to the consensus rate. 
% As our important result, 
% we compare the adversary tolerance ratio with the one in \cite{better_method,tighter_bound} , 
% and \cref{fig:final result} shows that our method can significantly promote the adversary tolerance ratio.


Furthermore, \cref{fig:adv_ratio: simulation vs theory} compares theoretical $\mathcal A$ with numerical simulation.
We can observe that the properties in \cref{prop:adversary ratio properties} still hold in simulation. 
The optimal \qname\ $q$ with respect to adversarial tolerance ratio $\mathcal{A}$ gradually decreases as $\theta$ ascends. 
It is also observable that $\mathcal{A}_\theta^*$ grows as $\theta$ grows. 
Compared with simulation data, theoretical results serve as relatively precise lower bounds for each case.
In theory, we always consider the worst cases, 
while simulation results are obtained in the sense of average. 
For example, a pattern `hh' is always assumed to cause a fork in theory, 
but it may not cause a fork in reality, 
because the two blocks may be mined by the same miner in consecutive time slots.
% JZ: do not find the following help. 
% However, the two blocks may be mined by the same miner in consecutive time slots, which will not cause a fork.

\def \green {ForestGreen}
\def \blue {RoyalBlue}
\def \orange {orange}
\def \marksquare {square}
\def \marko {o}
\def \marktri {triangle}

\begin{figure}[hbtp]
    \centering
\begin{tikzpicture}
    \begin{axis}[
        height = 0.5\textwidth,
        width = 0.45\textwidth,
        xlabel = \qname\ $ q $,   
        scaled ticks=false,
        ylabel = Adversary tolerance ratio $\mathcal{A}$,
        xmin=0.001,
        scaled ticks=false,
        xtick pos = left,
        ytick pos = left,
        x tick label style={/pgf/number format/.cd,std,precision=2,
                            /pgf/number format/fixed,     
                            /pgf/number format/fixed zerofill,
                             },
        legend style={at={(0.28,0.22)}, anchor=west, nodes={scale=1, transform shape}}
    ]
    
    \addplot [color=\blue , mark=\marksquare, thick ] table [x index=1,y index=4, col sep = comma] {tex_figure/adv_ratio/theta50.csv};
    % \addplot [color=\colorironw, mark=\markironw, thick] table [x index=1,y index=19, col sep = comma] {tex_figure/simulation/single-adv-0.csv};
    \addplot [color=red , mark=\marksquare , thick] table [x index=1,y index=4, col sep = comma] {tex_figure/adv_ratio/theta100.csv};
    \addplot [color=\green , mark=\marksquare , thick] table [x index=1,y index=4, col sep = comma] {tex_figure/adv_ratio/theta200.csv};
    \addplot [color=\orange , mark=\marksquare , thick] table [x index=1,y index=4, col sep = comma] {tex_figure/adv_ratio/theta400.csv};
    
    \addplot [color=\blue, dashed, thick] table [x index=1,y index=5, col sep = comma] {tex_figure/adv_ratio/theta50.csv};
    \addplot [color=red, dashed, thick] table [x index=1,y index=5, col sep = comma] {tex_figure/adv_ratio/theta100.csv};
    \addplot [color=\green, dashed, thick] table [x index=1,y index=5, col sep = comma] {tex_figure/adv_ratio/theta200.csv};
    \addplot [color=\orange, dashed, thick] table [x index=1,y index=5, col sep = comma] {tex_figure/adv_ratio/theta400.csv};
    % \legend{
    %     Ironclad(weight),
    %     Ironclad(size),
    %     Nakamoto(weight/size)
    %     }
    \legend{
        $\theta = 50$ in simulation,
        $\theta = 100$ in simulation,
        $\theta = 200$ in simulation,
        $\theta = 400$ in simulation,
    }
    \end{axis}
    
\end{tikzpicture}
    \caption{The adversary tolerance ratio $\mathcal{A}$ in theory and simulation with parameter settings: $p_h=\frac{3}{4\Delta}$, $\Delta=10^{13}$. 
    The dashed curves with the same colors correspond to theoretical results.
    The data points are computed by using the Definition \ref{def: tolerance ratio}, where the values of $\alpha$ are obtained from simulation with corresponding $\theta$ and $q$. 
    The simulation settings are explained in detail in \cref{section: Numerical Experiments}.
    }

    \label{fig:adv_ratio: simulation vs theory}
\end{figure}

% conjecture: 
% 1. large $\theta$, large tolerance  
% 2. $\theta=\infty$, $\frac{1}{p_h}+q\Delta < \frac{1}{p_a}$
% 3. $ q\to 0$, honest majority


==> attack/consensus_attack.tex <==

\subsection{Consensus Attack}
\label{subsec:consensus attack}

Suppose that the condition of \ref{thm: Consistency} is satisfied in our protocol, 
then according to \ref{rem: loose chain growth rate}, there exists $\gamma>0$ such that
\begin{equation}
    u = (1+\gamma)p_a (1-q+q\theta).
    \label{margin}
\end{equation}
The LHS is the chain growth rate $u$. 
Moreover, we reasonably assume that $\gamma$ is independent with $\theta$ and $q$, 
and only depends on the mining power and the network delay.
The confirmation time depends on the selection of parameters $\theta$ nad $q$.
The expression $S>\frac{\theta}{\gamma(q_a+\theta q_A)}$ indicates that a large $\theta$ requires long confirmation time.
We can establish a rigorous result in the sense of expectation by Wald's equation. Let 
$$
\tau = \min \left\{ t \bigg| \sum_{i=1}^{t} X_i < -\theta \right \}
$$
represent the minimum waiting time until the consensus attack fails. Hence, by Wald's equation \cite{sor},
$
\e{\tau} \e{X_i} < -\theta ,
$
so $$
\e{\tau} > \frac{\theta}{\gamma(q_a+\theta q_A)}.
$$


Since the honest will always admit the heaviest chain, the adversary have to provide a heavier chain in order to break the consistency.
In general, the adversary starts a consensus attack by forking from the head of the honest chain and mining a private chain.
The adversary will give up the attack when the weights of their private chain are less than those of the heaviest chain by $\theta$.
Intuitively, a larger $\theta$ may make a consensus attack easier to succeed, which causes a longer confirmation time.
To illustrate the effect of $\theta$ on the confirmation time, 
we compute the tail probability of successful attacks in the following lemma:

\begin{mylem}
    \label{lem:attack lemma}
Assume the honest parties adopt the chain $\chain_t$ at time slot $t$ and the mining power of two parties satisfies the relationship (\ref{margin}). 
If adversary parties start a consensus attack at the head of $\chain_t$ and form a private chain $\chain'_t$, 
then after $S$ consecutive time slots, the success probability is negligible in $S$. In other words,
$$
\prob{\diff{\chain'_{t+S}} > \diff{\chain_{t+S}} -\theta}\leq \exp\left(-{ \frac{ 2(\theta- S \gamma(q_a+\theta q_A) )^2  }{S\theta^2}  }\right)
$$
holds for $S>\frac{\theta}{\gamma(q_a+\theta q_A)}$.
\end{mylem}
Therefore, a large weight parameter $\theta$ requires more confirmation time in order to keep the security, 
which yields an upper bound for $\theta$ in terms of the confirmation time.
However, this model for adversary parties is still not precise.
We provide a more detailed one in the following subsection.


% An extreme case is $\theta \to +\infty$, 
% where the blockchain system is fragile with consensus attacks. 
% The attacker will only focus on the \BB s and spy on honest chains. 
% Once honest parties mine a \BB, the adversary give up this attack.
% However, when adversary parties mine a \BB\,
% they can publish their private chain at a proper time slot to confuse honest parties and thus break the consistency.
% Since the probability of obtaining a \BB\ is a constant, the consensus attack will finally succeed with high probability. 
% The same holds for sufficiently large $\theta$.
% From the argument above, the fragility occurs as the cost and the reward for obtaining a \BB\ is imbalanced. 
% The adversary may benefit a lot from an overlarge $\theta$ at a low cost $q_A$.





==> attack/random_walk.tex <==



\subsection{A Random Walk Model for Attacks}
\label{subsec: random walk}
In the subsection \ref{subsec:consensus attack}, 
we apply the concentration inequality and Wald's equation to reveal the relationship between the confirmation time and weight parameter $\theta$.
This result makes sense in expectation but is not precise enough to capture attack details.

We first build a random walk model to capture the features of adversary attacks.
The blockchain state is a point $(X,Y)$ in a plane representing that the heaviest chain leads the adversary chain by $X$ \SB s and $Y$ \BB s. 
The adversary parties start an attack on the head of the heaviest chain, 
so the initial starting point is $(0,0)$.
At the time slot $t$, the blockchain system will generate a tuple of random variables $(X_t,Y_t)$.
The sequence of these random variables is determined by 
$$
X_{t+1} = \left \{
\begin{array}{lcl}
X_{t} + 1, \text{with probability } \frac{u}{1-q+q\theta}(1-q')(1-p_a(1-q)),\\
X_{t} - 1, \text{with probability } (1-\frac{u}{1-q+q\theta}(1-q'))p_a(1-q),\\
X_t, \text{others},\\
\end{array}
\right.
$$
and 
$$
Y_{t+1} = \left \{
\begin{array}{lcl}
Y_{t} + 1, \text{with probability } \frac{u}{1-q+q\theta}q'(1-p_aq),\\
Y_{t} - 1, \text{with probability } (1-\frac{u}{1-q+q\theta}q')p_aq,\\
Y_t, \text{others},\\
\end{array}
\right.
$$
where $q'$ is the probability that a \BB occurs in the heaviest chain. 
Denote the stopping time, namely, the time when adversary parties consider their attack to fail, as 
$$
\tau = \{t: X_t +\theta Y_t \geq \text{threshold} \}.
$$
\bgmlover{should define a general function}
If the heaviest chain lead $\theta$ weights, 
it will be suitable for the adversary to switch to the heaviest chain and start a new attack.
Hence, We set the threshold to be $\theta$ for this attack in advance, 
and if the leading weights are larger than $\theta$, the attack is considered to fail.
During the random walk, the meaningful messages are the distributions of the following statistics:
$$
\text{maximal fork length(MFL)} = \max \{  - X_t - Y_t| t \leq \tau \},
$$
and 
$$
\text{maximal fork weights(MFW)} = \max \{  - X_t - \theta Y_t| t \leq \tau \}.
$$

However, this time-based model induces many technical challenges. 
For one thing, a sufficiently long period consists of extremely numerous time slots, 
which is too time-consuming to solve by computers. 
Moreover, no block is produced in the majority of time slots, 
which is a waste of resources in simulation.
For another, it is intractable to solve this random sequence to obtain a closed-form solution,
due to the difficult nature of this problem and the unavailability of parameters $u$ and $q'$.

To tackle the first challenge, we transfer this time-based model to an event-driven one. 
Once a block is generated, we randomly make it honest or adversary and then determine its type according to conditional probabilities, $q$ and $1-q$.
Once honest parties generate a block, the corresponding coordinate will increase by $1$.
If adversary parties produce a new block, the counterpart will decrease.
Each event about block production will make the blockchain state move from one point to another.
The value of $q'$ is not available in theory unless estimated by real-world data.
Intuitively, $q'>q$ because \BB s have more chances of admission by the heaviest chain.
Hence, we plug in $q$ in this random walk model to address the second challenge, 
which induces an upper bound for the attack success probability.
We reformulate the random sequence in this way:
$$
(X'_{n+1},Y'_{n+1} ) = \left \{
\begin{array}{lcl}
(X'_{n} + 1, Y'_n), \text{with probability } \frac{(1+\gamma)(1-q)}{2+\gamma} ,\\
(X'_{n} - 1, Y'_n), \text{with probability } \frac{1-q}{2+\gamma},\\
(X'_{n}, Y'_n + 1), \text{with probability } \frac{(1+\gamma)q}{2+\gamma},\\
(X'_{n}, Y'_n - 1), \text{with probability } \frac{q}{2+\gamma},\\
\end{array}
\right.
$$
where $\gamma$ satisfies $u = (1+\gamma) p_a(1-q+q\theta)$. 
The parameter $\gamma$ can be considered as the mining gap and determined in advance.
Then, we explain the probability of each transition and take the first transition as an example.
The probability of honest blocks occurrence is proportional to chain growth rate $u=(1+\gamma) p_a$, 
and the block to be a \SBs is proportional to $1-q$. 
Therefore, the first probability is proportional to $(1+\gamma)(1-q)$. 
Following the above reasoning, we get above four probabilities.
One may worry about the case that two blocks are produced in the same time slot.
This challenge can be addressed by sorting.
We sort events by their timestamps at first. 
If two blocks share the same timestamp, the algorithm should deal with the adversary block at first.
This trick shows preference to adversary parties and thus leads to an upper bound for success attack probability.

\bgmlover{Can it be called Monte Carlo?}
We apply the Monte Carlo algorithm to solve the new problem,
which is an easy way to obtain numerical solutions. 
During each attack, the Monte Carlo algorithm samples a path from the origin to the point which is beyond the area of halfplane $\{(x,y)|x +\theta y < \text{threshold}\}$.
Another advantage is that this algorithm can estimate the distributions of two statistics, 
which are of great importance to analyze their tail probabilities. 

From the numerical experiments, we can find that the adversary parties can hold 
one, two, and more than three \BB (s) with probability $4.7\%,0.3\%$ and $0.06\%$ for each.







==> discussion/consensus_attack.tex <==

\subsection{Consensus Attack}
\label{consensus attack}

Suppose that the condition of \ref{thm: Consistency} is satisfied in our protocol, then 
according to \ref{rem: loose chain growth rate}, there exists $\gamma>0$ such that
\begin{equation}
    u \geq (1+\gamma)p_a (1-q+q\theta).
    \label{margin}
\end{equation}
The LHS is the chain growth rate $u$. 
Moreover, we reasonably assume that $\gamma$ is independent with $\theta$ and $q$, 
and only depends on the mining power and the network delay.

Since the honest will always admit the heaviest chain,  the adversary have to provide a heavier chain in order to break the consistency.
In general, the adversary starts a consensus attack by forking from the head of the honest chain and mining a private chain.
The adversary will give up the attack when the weights of their private chain are less than those of the heaviest chain by $\theta$.
Intuitively, a larger $\theta$ may make a consensus attack easier to succeed, which causes a longer confirmation time.
To illustrate the effect of $\theta$ on the confirmation time, we compute the probability of successful attacks in the following lemma:


\begin{mylem}
Assume the honest parties adopt the chain $\chain_t$ at time slot $t$ and the mining power of two parties satisfies the relationship (\ref{margin}). 
If adversary parties start a consensus attack at the head of $\chain_t$ and form a private chain $\chain'_t$, 
then after $S$ consecutive time slots, the success probability is negligible in $S$. In other words,
$$
\prob{\diff{\chain'_{t+S}} > \diff{\chain_{t+S}} -\theta}\leq \exp\left(-{ \frac{ 2(\theta- S \gamma(q_a+\theta q_A) )^2  }{S\theta^2}  }\right)
$$
holds for $S>\frac{\theta}{\gamma(q_a+\theta q_A)}$.
\end{mylem}

\begin{myproof}
Denote the random variable $X_i$ as the weight advantage between adversary and honest parties at time slot $i$. 
Then,
$$
\e{X_i} = -\gamma p_a (1-q+q\theta).
$$
Obviously, $X_i$ is a bounded random variable since each party can only obtain at most one PoW at any time slot. 
Hence, $|X_i|\leq \theta$.

Without loss of the generality, assume the attack starts at time slot $1$. 
Then, $\sum_{i=1}^S X_i$ represents the weight advantage after $S$ time slots. 
We have
$$
\begin{array}{rcl}
& &\prob{\diff{\chain'_{t+S}} > \diff{\chain_{t+S}} -\theta}\\
& = & \prob{ \sum_{i=1}^S X_i >-\theta } \\
& = & \prob{ \sum_{i=1}^S X_i - S\e{X_i} >-\theta- S\e{X_i} } \\
& \leq & \exp(-{ \frac{ 2(\theta+S\e{X_i})^2  }{S\theta^2}  }) \\
& = &   \exp(-{ \frac{ 2(\theta- S \gamma(q_a+\theta q_A)   )^2  }{S\theta^2}  }) 
\end{array}
$$
for $S>\frac{\theta}{\gamma(q_a+\theta q_A)}$.
The last inequality is from the McDiarmid’s inequality. 
The RHS quickly converges to zero as $S$ goes to infinity, 
so the consensus attack succeeds with negligible probability.

% \textcolor{orange}{Check again}
% If $S>\frac{2\theta}{\gamma(q_a+\theta q_A)}$, then the RHS can be simplified as
% $$
% \begin{array}{rcl}
% \exp(-{ 2\frac{ (\theta+S\e{X_i})^2  }{S\theta^2}  })
% &\leq& \exp(-{ \frac{S \e{X_i}^2}{\theta^2}  }) \\
% &\leq& \exp(-\frac{S\gamma^2(q_a+\theta q_A)^2  }{\theta^2} )\\
% &\leq& \exp(-{S\gamma^2 q_A^2 } )
% \end{array}
% $$

\end{myproof}

\begin{myrem}
The expression $S>\frac{\theta}{\gamma(q_a+\theta q_A)}$ indicates that a large $\theta$ requires long confirmation time.
We can establish a more rigorous result in the sense of expectation. Let 
$$
\tau = \min \left\{ t \bigg| \sum_{i=1}^{t} X_i < -\theta \right \}
$$
represent the minimum waiting time until the consensus attack fails. Hence, by Wald's equation \cite{sor},
$
\e{\tau} \e{X_i} < -\theta ,
$
so $$
\e{\tau} > \frac{\theta}{\gamma(q_a+\theta q_A)}.
$$
\end{myrem}


Therefore, a large weight parameter $\theta$ requires more confirmation time in order to keep the security, 
which yields an upper bound for $\theta$ in terms of the confirmation time.
% An extreme case is $\theta \to +\infty$, 
% where the blockchain system is fragile with consensus attacks. 
% The attacker will only focus on the \BB s and spy on honest chains. 
% Once honest parties mine a \BB, the adversary give up this attack.
% However, when adversary parties mine a \BB\,
% they can publish their private chain at a proper time slot to confuse honest parties and thus break the consistency.
% Since the probability of obtaining a \BB\ is a constant, the consensus attack will finally succeed with high probability. 
% The same holds for sufficiently large $\theta$.
% From the argument above, the fragility occurs as the cost and the reward for obtaining a \BB\ is imbalanced. 
% The adversary may benefit a lot from an overlarge $\theta$ at a low cost $q_A$.





==> growth_and_quality.tex <==

\section{Chain Growth and Chain Quality} 
\label{section:growth and quality}


We begin with the chain growth property in the $\Delta$-fork. 
The following value reflects the weight growth rate in the heaviest chain, 
though the heaviest chain in the fork may differ at each time slot. 
The weight growth rate is also vital for security analysis.




\begin{mylem} \label{chain growth}
Given $S\in [L]$, $t \in[L-S]$ and a  $\Delta$-fork $F_t$ over a lifetime of $L$ slots, then for any $\delta>0$,  
$\diffFC{t+S}-\diffFC{t}$ is at least $(1-\delta)S p_h\frac{1-q+q\theta}{1+p_h\Delta}$  
with probability $1-e^{\Omega(-S{\delta}^2)}$.
\end{mylem}

\begin{myproof}
At the time slot $t$, each honest player will try to extend a path whose weight is at least $\diffFC{t}$, 
because at time $t-\Delta$, the heaviest path has weight $\diffFC{t}$ and after $\Delta$ rounds, 
every honest party will hold a chain with weight at least $\diffFC{t}$. 

Let $\tau$ denote the time interval such that 
$$
\tau = \min\{t':\diffFC{t+t'}\geq \diffFC{t}+(1-q)+q\theta \},
$$
then $\e{\tau} \leq \frac{1}{p_h}+\Delta$. The expected weight of a block is $(1-q)+q\theta$, and 
the expected time to produce a block for honest parties is $\frac{1}{p_h}$. Therefore, after $\Delta$ time slots, 
each honest party will hold a chain with weight at least $\diffFC{t+\tau}$ at time $t+\tau$. 
Then we conclude that in the sense of expectation, 
one will extend a block to the heaviest chain in $F_t$ with time interval at most $\frac{1}{p_h}+\Delta$. 
Then for $S$ rounds, the heaviest chain will increase weight at least 
$$
S p_h\frac{1-q+q\theta}{1+p_h\Delta},
$$
and this indicates $\diffFC{t+S}\geq S p_h\frac{1-q+q\theta}{1+p_h\Delta}$ in the sense of expectation. 
We finish the proof by applying the Hoeffding's inequality:
$$
\diffFC{t+S}-\diffFC{t}\geq (1-\delta)S p_h\frac{1-q+q\theta}{1+p_h\Delta}
$$
with probability $1-e^{\Omega(-S{\delta}^2)}$.
\end{myproof}

\begin{mycol}
Our protocol satisfy the chain growth property with growth rate parameter $u=\frac{p_h(1-q+q\theta)}{1+p_h\Delta}$.
\end{mycol}

\begin{myrem}
    \label{rem: loose chain growth rate}
    From the proof of the lemma \ref{chain growth}, we can see the bound for $\e{\tau}$ is loose for some cases. 
    When $p_h\approx 1$, $\e{\tau}$ is much less than $\Delta$. 
    Therefore, the chain growth rate derived in the lemma \ref{chain growth} is not tight.
    Theoretically, the chain growth rate $u$ should be larger than the consensus rate $\alpha$, 
    because there are a proportion of weights from the blocks which do not lead to consensus in the heaviest chain.
    However, $u$ is less than $\alpha$ for specific parameters, 
    e.g., $p_h=2\times 10^{-13},\Delta = 10^{13},q=0.02,\theta=500$.
\end{myrem}

Next, we consider the chain quality which reflects the fraction of the honest cumulative weights in the heaviest chain.

The following lemma computes the cumulative weights produced by the adversary in a given period, 
and the value will not deviate from its mean with overwhelming probability.

\begin{mylem} \label{adv upper bound}
Let $D_t$ denote the cumulative weights of blocks mined by adversary parties during $t$ time slots, then for any $\delta>0$,
$$
\prob{D_t >(1+\delta)p_at(1-q+q\theta) }\leq \exp(-\Omega(\delta^2t)).
$$
\end{mylem}
\begin{myproof}
WLOG, we can assume the beginning time slot is $1$. 
Let random variable $X_i$ denote the weights contributed by the adversary at slot $i\in[t]$. 
The probability mass function of $X_i$ is 
$$
\prob{X_i=1}=q_a , \prob{X_i=\theta}=q_A, \prob{X_i=0}=1-p_a.
$$
Since $X_i$ is a bounded random variable, then
$$
\begin{array}{rcl}
& & \prob{D_t\geq(1+\delta)t p_a(1-q+q\theta)}\\&=&\prob{\sum_{i=1}^t X_i \geq(1+\delta)t \e{X_i}}\\ &\leq& \exp({-\Omega(\delta^2t)}),
\end{array}
$$
where the last inequality is directly from the Hoeffding's inequality.
\end{myproof}


\begin{mylem}
For a $\Delta$-fork $F_t$ over a lifetime of $L$ slots, consider a chain $\chain_{t-\Delta} \subset \closure{t}$ such that 
$\diff{\chain_{t-\Delta}} = \diffFC{t}$. 
For any suffix path $\mathcal{S}\subset\chain_{t-\Delta}$ of the chain with the cumulative weight $D$, 
if the first block in $\mathcal{S}$ is honest and shares the same last block with $\chain_{t-\Delta}$, 
then for every $\delta >0$, the fraction of weights contributed by honest blocks in $\mathcal{S}$ is at least 
$1-(1+\delta)(\frac{p_a}{p_h}+p_a \Delta)$ with probability $1-e^{-\Omega(\delta^2D)}$.
\end{mylem}

\begin{myproof}
Suppose $\mathcal{S}\subset \chain_{t-\Delta}$ starts with an honest block $B$ whose label is $t_1$ 
and the cumulative weight of $\mathcal{S}$ is $D$, then it suffices to show that 
the weight contributed by adversary blocks is at most $(1+\delta)(\frac{p_a}{p_h}+p_a \Delta)D$ in $\mathcal{S}$ 
with high probability for every $\delta>0$. 

Since $B$ is honest, then we have $\diff{\chain_{t_1}} \leq \diff{ \overline{ F_{t_1}} }$ 
according to the definition of the maximal honest subfork. 
Thus, by Lemma \ref{chain growth}, for every $\delta_1>0$, 
the chain growth rate of the this segment is at least $(1-\delta_1)p_h \frac{1-q+q\theta}{1+p_h\Delta}$ 
except with probability $\exp({-\Omega(\delta_1^2D)})$. Then
$$
t-\Delta-t_1\leq \frac{D(1+p_h\Delta)}{(1-\delta_1)(1-q+q\theta)p_h}.
$$

By Lemma \ref{adv upper bound}, for every $\delta_2>0$, 
the weights contributed by adversary blocks in the time interval are upper bounded by 
$$
(1+\delta_2)p_a (t-\Delta-t_1)(1-q+q\theta) \leq \frac{(1+\delta_2)(\frac{p_a}{p_h}+p_a\Delta) D}{(1-\delta_1)}
$$
except with probability $e^{-\Omega(\delta_1^2D)}+e^{-\Omega(\frac{\delta_2^2}{1-\delta_1}D)}$.

For a given $\delta >0$, we can select a $\delta_1$ and let $1+\delta = \frac{1+\delta_2}{1-\delta_1}$, 
so the fraction of the cumulative weights contributed by adversary parties are at most 
$(1+\delta)(\frac{p_a}{p_h}+p_a \Delta)$ except with probability $\exp({-\Omega(\delta^2D)})$.
\end{myproof}



\begin{mycol}
Our protocol satisfies the chain quality property with quality parameter 
$f = 1-(1+\delta)(\frac{p_a}{p_h}+p_a \Delta)$ with high probability.
\end{mycol}

\begin{myrem}
From the chain quality property, we obtain a loose bound for the adversary mining power: 
$$
\frac{p_a}{p_h}+p_a \Delta<1 \Leftrightarrow \frac{1}{p_h}+\Delta < \frac{1}{p_a}.
$$
In order to maintain the chain quality, 
the average mining time for honest parties plus delay should be less than the average mining time for adversary parties. 
It is also the theoretical upper bound to maintain the consistency in the model without \BB s, seen in \cite{tighter_bound}. 
Namely, if the adversary mining power exceeds the threshold provided by the above inequality, 
the blockchain system is not secure for consensus attacks. 
However, since we introduce \BB s in our protocol, 
this bound cannot be directly applied to our model. 
Our protocol can tolerate more adversary mining power.
% Furthermore, it is unnecessary to approach the bound in practice  
% because the properties of the blockchain system will be heavily damaged at the boundary. 
\end{myrem}




==> matlab_result/expressions.tex <==
% adversary power in terms of honest power with difficult block
% adv_hon_ratio = ((H + h*(1 - h - H)^d)*(h*(1 - h - H)^d + H*w*(1 - H)^d)*(1 - H)^d)/((H + h)*(h + H*w))

% % adversary power in terms of honest power without difficult block
% adv_hon_ratio_h = (1 - h - H)^(2*d)

% % the improvement 
% ratio = adv_hon_ratio / adv_hon_ratio_h = ((H + h*(1 - h - H)^d)*(h*(1 - h - H)^d + H*w*(1 - H)^d)*(1 - H)^d/(1 - h - H)^(2*d))/((H + h)*(h + H*w))



==> security_analysis.tex <==


\subsection{selection of } 
\label{section: Security}

%\input{../../tex/journal/attack/consensus_attack.tex}

\input{./random_walk.tex}

%\input{../../tex/journal/discussion/discussion_parameters.tex}


% In \cref{subsec:consensus attack} and \cref{subsec: random walk}, we present a detailed analysis of protocols with our method under a consensus attack, 
% deriving bounds on the probability that the weights of an adversarial chain exceed the weights of the current heaviest honest chain minus $\theta$,
% thus yielding an upper bound of $\theta$. 
% The security analysis also shows a trade-off between consistency and confirmation time.

%%%%%%%%%% numerical results for q* %%%%%%%%%%
%%%%%   ph=1e-13，delta=1e13
% theta = 1000,q^* = 0.02275 
% theta = 500, q^* = 0.0271875
% theta = 200, q^* = 0.0438125
% theta = 100, q^* = 0.06375
% theta = 50,  q^* = 0.08375


%%%%%%%%%% numerical results for q* %%%%%%%%%%
%%%%%   ph=1e-13/60，delta=1e13
% theta = 1000,q^* = 0.03325
% theta = 500, q^* = 0.03325    % almost same as theta = 1000
% theta = 200, q^* = 0.03325  
% theta = 100, q^* = 0.099875
% theta = 50,  q^* = 0.099875


%%%%%%%%%% numerical results for q* %%%%%%%%%%
%%%%%   p=1e-13, delta=1e13, p_h = 0.75*p
% theta = 1000,q^* = 0.0199375

% theta = 500, q^* = 0.03175    
% theta = 200, q^* = 0.048  
% theta = 100, q^* = 0.07175
% theta = 50,  q^* = 0.088


%%%%%%%%%% numerical results for q* %%%%%%%%%%
%%%%%   p=1e-13, delta=1e13, p_h = 0.51*p
% theta = 1000,q^* = 0.02275
% theta = 500, q^* = 0.035875 
% theta = 200, q^* = 0.051125
% theta = 100, q^* = 0.070625
% theta = 50,  q^* = 0.09675


%%%%%%%%%% numerical results for q* %%%%%%%%%%
%%%%%   p=1e-13/60, delta=1e13, p_h = 0.75*p
% theta = 1000,q^* = 0.044375    % almost same
% theta = 500, q^* = 0.044375    % almost same
% theta = 200, q^* = 0.044375    % almost same
% theta = 100, q^* = 0.044375    % almost same
% theta = 50,  q^* = 0.133125


%%%%%%%%% numerical results for q* %%%%%%%%%%
%%%%%   p=1e-13/60, delta=1e13, p_h = 0.51*p
% theta = 1000,q^* = 0.06525    % almost same
% theta = 500, q^* = 0.06525    % almost same
% theta = 200, q^* = 0.06525    % almost same
% theta = 100, q^* = 0.06525    % almost same
% theta = 50,  q^* = 0.06525    % almost same

%%%%%%%%%%  numerical results for theta %%%%%%%%%%
%%%%%   ph=1e-13/60，delta=1e13, eps = 1e-10
% q = 1e-6 : theta > 46.15160552860578
% q = 1e-3 : theta > 46.15150582050343
% theta > 46.15160562841359 for any q in (0,1) % q = 0 

%%%%%   ph=1e-13，delta=1e13, eps = 1e-10
% q = 1e-6 : theta > 51.75404442235177
% q = 1e-3 : theta > 51.74860371981532
% theta > 51.75404986827829 for any q in (0,1) % q = 0 


%%%%%   ph=1e-12，delta=1e13, eps = 1e-10
% q = 1e-6 : theta > 91.73164211685122
% q = 1e-3 : theta > 91.69276721520836
% theta > 91.73168102699431 for any q in (0,1) % q = 0 


%%%%%   ph=1e-13，delta=1e13, eps = 1e-5
% q = 1e-6 : theta > 28.501277756830227
% q = 1e-3 : theta > 28.496210016089105
% theta > 28.5012828293288 for any q in (0,1) % q = 0 

% the dominant terms in expression are  Delta * ph, log(eps^-1).
